Prompt engineering and its implications on the energy consumption of Large Language Models

Reducing the environmental impact of AI-based software systems has become critical. The intensive use of large language models (LLMs) in software engineering poses severe challenges regarding computational resources, data centers, and carbon emissions. In this paper, we investigate how prompt engineering techniques (PETs) can impact the carbon emission of the Llama 3 model for the code generation task. We experimented with the CodeXGLUE benchmark to evaluate both energy consumption and the accuracy of the generated code using an isolated testing environment. Our initial results show that the energy consumption of LLMs can be reduced by using specific tags that distinguish different prompt parts. Even though a more in-depth evaluation is needed to confirm our findings, this work suggests that prompt engineering can reduce LLMs' energy consumption during the inference phase without compromising performance, paving the way for further investigations.

==> tab/rq1.tex <==
\begin{table}[]
\caption{Energy Consumption of the different PETs using the configuration a.}
\label{tab:rq1}
\centering
\small
\begin{tabular}{lllll}
\cline{2-4}
\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{Consumption in kWh}} &  \\ \cline{1-4}
\multicolumn{1}{|l|}{\textbf{Configuration}} & \multicolumn{1}{l|}{\textbf{Zero-Shot}} & \multicolumn{1}{l|}{\textbf{One-Shot}} & \multicolumn{1}{l|}{\textbf{Few-Shot}} &  \\ \cline{1-4}
\multicolumn{1}{|l|}{Configuration a} & \multicolumn{1}{l|}{0.0000157} & \multicolumn{1}{l|}{0.0000347} & \multicolumn{1}{l|}{0.0000537} &  \\ \cline{1-4}
 &  &  &  &  \\
 &  &  &  & 
\end{tabular}
\end{table}
